Multimodal Diffusion Transformer: Learning Versatile Behavior from Multimodal Goals

This work introduces the Multimodal Diffusion Transformer (MDT), a novel diffusion policy framework, that excels at learning versatile behavior from multimodal goal specifications with few language annotations. MDT leverages a diffusion-based multimodal transformer backbone and two self-supervised auxiliary objectives to master long-horizon manipulation tasks based on multimodal goals. The vast majority of imitation learning methods only learn from individual goal modalities, e.g. either language or goal images. However, existing large-scale imitation learning datasets are only partially labeled with language annotations, which prohibits current methods from learning language conditioned behavior from these datasets. MDT addresses this challenge by introducing a latent goal-conditioned state representation that is simultaneously trained on multimodal goal instructions. This state representation aligns image and language based goal embeddings and encodes sufficient information to predict future states. The representation is trained via two self-supervised auxiliary objectives, enhancing the performance of the presented transformer backbone. MDT shows exceptional performance on 164 tasks provided by the challenging CALVIN and LIBERO benchmarks, including a LIBERO version that contains less than $2\%$ language annotations. Furthermore, MDT establishes a new record on the CALVIN manipulation challenge, demonstrating an absolute performance improvement of $15\%$ over prior state-of-the-art methods that require large-scale pretraining and contain $10\times$ more learnable parameters. MDT shows its ability to solve long-horizon manipulation from sparsely annotated data in both simulated and real-world environments. Demonstrations and Code are available at https://intuitive-robots.github.io/mdt_policy/.

==> chapters/evaluation.tex <==

\section{Evaluation}

\input{tables/calvin_main_table}
This section aims to answer the following questions:
\begin{itemize}
    \item (I) Is \gls{mdt} able to learn long-horizon manipulation from play data with few language annotations?
    \item (IIa) Do Masked Generative Foresight and Contrastive Latent Alignment enhance the performance of \gls{mdt}? 
    \item (IIb) Does \gls{mgf} improve the performance of other transformer policies?
    \item (III) Can \gls{mdt} learn language-guided manipulation from partially labeled data in a real-world setting?
    % \item (IV) Which are the key components of MDT and the self-supervised losses to enable effective language understanding with limited annotations?
\end{itemize}



\subsection{Simulated Benchmark Environments}

\begin{table*}[h!]
\centering
\scalebox{0.95}{
\begin{tabular}{l|c|cc|cccccc}
\toprule
Method & Language Annotation & $\mathcal{L}_{\text{CLA}}$ & $\mathcal{L}_{\text{MGF}}$ & Spatial & Object & Goal  & Long & 90 & Average  \\ 
\midrule
Transformer-BC~\cite{liu2023libero} & 100 $\%$ & $\times$ &  $\times$&  71.83 $\pm$ 3.7 & 71.00 $\pm$ 7.9 & $76.33 \pm 1.3$ &  $24.17 \pm 2.6$ & - & -  \\
\midrule
 Distill-D & $2\%$ & $\times$ & $\times$ & $46.8\pm2.8$   & $72.0 \pm 6.5$   & $63.8 \pm 2.5$ & $47.3 \pm 4.1$ & $49.9 \pm 1.0$  & $56.0 \pm 3.4$ \\
\midrule
\multirow{4}{*}{MDT}  & $2\%$ & $\times$ & $\times$ & $66.0 \pm 1.9$   & $85.2 \pm 2.3$   & $67.8 \pm 4.6$ & \textbf{65.0} $\pm$ \textbf{2.0} & $58.7 \pm 0.8$  & $68.8 \pm 2.2$ \\
% CLIP Only
& $2\%$ & $\checkmark$ & $\times$ & $74.3 \pm 0.8$   & $87.5 \pm 2.7$   & $71.5 \pm 3.5$ &  $63.9 \pm 4.5$ & $66.9 \pm 1.7$  &  \textbf{72.8} $\pm$ \textbf{2.6} \\
% MGF only
& $2\%$ & $\times$ & $\checkmark$ &  $67.5 \pm 2.1$   & $87.5 \pm 2.6$   & $69.3 \pm 2.5$ &  $61.8 \pm 2.5$ & $62.6 \pm 1.0$  & $69.7 \pm 2.1$ \\
% both
&  $2\%$ & $\checkmark$ & $\checkmark$ & \textbf{78.5} $\pm$ \textbf{1.5}  & \textbf{87.5} $\pm$ \textbf{0.9}   & \textbf{73.5} $\pm$ \textbf{2.0} & $57.1 \pm 0.8$ & \textbf{67.2} $\pm$ \textbf{1.1} & $72.5 \pm 1.5$ \\ 
\bottomrule
\end{tabular}
}
\caption{Overview of the performance of MDT and baselines with and without our proposed Self-Supervised Losses on several LIBERO Task suites. 
All results show the average performance of all tasks averaged over 20 rollouts each and with 3 seeds. 
MDT does outperform the Transformer-BC baseline in several settings with only $2\%$ of language annotations.}
\label{tab: libero ablations}
\end{table*}
We conduct multiple simulation experiments on two popular and challenging robot learning benchmarks:

\textbf{CALVIN.}
The CALVIN challenge~\cite{mees2022calvin} 
% has been designed to assess the performance of robot manipulation policies that are conditioned on language, particularly for tasks requiring extended planning and execution horizons.
consists of four similar but different environments A, B, C, D. 
The four setups vary in desk shades and the layout of items as visualized in \autoref{fig: sim_overview}.
The main experiments for this benchmark are conducted on the full dataset ABCD$\rightarrow$D, where the policies are trained on ABCD and evaluated on D. 
This setting contains $24$ hours of uncurated teleoperated play data with multiple sensor modalities and $34$ different tasks for the model to learn. 
Further, only $1\%$ of data is annotated with language descriptions.
All methods are evaluated on the long-horizon benchmark, which consists of $1000$ unique sequences of instruction chains, described in natural language. 
Every sequence requires the robot to continuously solve $5$ tasks in a row.
%each containing demonstrations of $5$ tasks that are described in natural language.
During the rollouts, the agent gets a reward of $1$ for completing the instruction with a maximum of $5$ for every rollout.
We additionally perform experiments on the small benchmark D$\rightarrow$D consisting of only 6 hours of play data.

\textbf{LIBERO.} We further evaluate various models on LIBERO~\cite{liu2023libero}, a robot learning benchmark consisting of over 130 language-conditioned manipulation tasks divided into $5$ different task suites, with different foci. 
Details are provided in \autoref{sec: libero} of the Appendix. 
Every task in each suite has $50$ demonstrations, where we only label one demonstration with the associated task description and all others without.
During evaluation, we test all models on all tasks with 20 rollouts each and average the results over 3 seeds.
During the experiments, we restrict all policies to only use a static camera and a wrist-mounted one. 

\subsection{Baselines}

We compare our proposed policy against the following state-of-the-art language-conditioned multi-task policies on CALVIN:
\begin{itemize}
    \item \textbf{HULC:} A hierarchical play policy, that uses discrete \gls{vae} skill space with an improved low-level action policy and a transformer plan encoder to learn latent skills \cite{mees2022hulc}.
    \item \textbf{LAD:} A hierarchical diffusion policy, that extends the HULC policy by substituting the high-level planner with a U-Net Diffusion model~\cite{zhang2022lad} to diffuse plans. 
    \item \textbf{Distill-D:} A language-guided Diffusion policy from~\cite{ha2023scaling}, that extends the initial U-Net diffusion policy~\cite{chi2023diffusionpolicy} with additional Clip Encoder for language-goals. 
    We use our continuous time diffusion variant instead of the discrete one for direct comparison and extend it with the same CLIP vision encoder to guarantee a fair comparison. 
    \item \textbf{MT-ACT:} A multitask transformer policy~\cite{bharadhwaj2023roboagent, zhao2023learning}, that uses a \gls{vae} encoder for action sequences and also predicts action chunks instead of single actions with a transformer encoder-decoder architecture. 
    \item \textbf{RoboFlamingo:} A finetuned Vision-Language Foundation model \cite{li2023vision} containing $3$ billion parameters, that has an additional recurrent policy head for action prediction.
    The model was pretrained on a large internet-scale set of image and text data and then finetuned for CALVIN. 
    % For behavior generation all $32$ cross-attention layers and the additional policy head were finetuned that contains approx. 1 billion trainable parameters. 
\end{itemize}
We adopt the recommended hyperparameters for all baselines to guarantee a fair comparison and give an overview of our chosen hyperparameters for self-implemented baselines in Appendix~\ref{sec: baseline Implementations}.
Further, we directly compare the self-reported results of HULC, LAD, and RoboFlamingo on CALVIN \cite{zhang2022lad, mees2022hulc, li2023vision, zhang2022lad}. 
All models use the same language and image goal models to further ensure fair comparisons.
Since RoboFlamingo only published the best seed of each model, we can not include standard deviations in their results.
For our experiments in LIBERO, we report the performance of MDT, Distill-D, and the best transformer baseline policy from the original benchmark, which was trained with full language annotations \cite{liu2023libero}.

\subsection{Evaluation Results}

\begin{table}[]
    \centering
    \begin{tabular}{l|c}
        Policy & Avg. Len. CALVIN  \\
         \midrule
        MT-ACT & 2.80 $\pm$ 0.03 \\
        MT-ACT + $\mathcal{L}_{\text{MGF}}$ & \textbf{4.03} $\pm$ \textbf{0.08} \\ 
    \bottomrule
    \end{tabular}
    \caption{Evaluation of the Performance Increase of the MT-ACT policy with the additional Masked Generative Foresight Loss on the CALVIN ABCD$\rightarrow$D challenge.}
    \label{tab: MT-ACT Ablations}
\end{table}


\begin{table*}[]
    \centering
    \begin{tabular}{l|l|ccccc|c}
    Goal Modality  & Model & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Avg. Rollout Length  \\
        \midrule
  \multirow{3}{*}{Language}    & MT-ACT   & 50\% & 50\% & 0\% & 0\% & 0\% & 1.00 $\pm$ (1.00) \\
     & MDT      & 40\% & 40\% & 0\% & 0\% & 0\% & 0.80 $\pm$ (0.98) \\
     % & MDT-V    & 60\% & 60\% & 60\% & 20\% & 0\% & 2.00 \\
     & MDT + $\mathcal{L}_{\text{MGF}}$ & 90\% & 80\% & 10\% & 0\% & 0\% &  \textbf{1.80 $\pm$ (0.75)} \\
     \midrule
 \multirow{3}{*}{Images}      & MT-ACT   & 50\% & 40\% & 20\% & 10\% & 0\% & 1.20 $\pm$ (1.40) \\
     & MDT      & 60\% & 30\% & 30\% & 10\% & 0\% & 1.30 $\pm$ (1.42) \\
     % & MDT-V    & 80\% & 80\% & 40\% & 40\% & 0\% & 2.4 \\
     & MDT + $\mathcal{L}_{\text{MGF}}$ & 100\% & 90\% & 90\% & 0\% & 0\% & \textbf{2.80 $\pm$ (0.60)} \\
      \bottomrule
    \end{tabular}
    \caption{Average rollout length of different policies evaluated in our real robot play kitchen. We present the average performance of various policies tested on 10 long horizon instruction chains.}
    \label{tab: real robot experiments}
\end{table*}
The results of all our experiments on CALVIN are summarized in Table~\ref{tab: CALVIN Long horizon}. 
We assess the performance of \gls{mdt} and \gls{mdt}-V on ABCD$\rightarrow$D and on the small subset D$\rightarrow$D.
The results are shown in \autoref{tab: CALVIN Long horizon}. 
\gls{mdt}-V sets a new record in the CALVIN challenge, extending the average rollout length to $4.51$ which is a $10\%$ absolute improvement over RoboFlamingo. 
\gls{mdt} also surpasses all other tested methods.
Notably, \gls{mdt} achieves this while having less than $10\%$ of trainable parameters and not requiring pretraining on large-scale datasets. 
In the scaled-down CALVIN D$\rightarrow$D benchmark, \gls{mdt}-V establishes a new standard, outperforming recent methods like LAD~\cite{zhang2022lad} and boosting the average rollout length by $20\%$ over the second best baseline.
While RoboFlamingo demonstrates commendable performance on the complete ABCD dataset, it relies on substantial training data and remains untested on the D$\rightarrow$D subset. In contrast, \gls{mdt} excels in both scenarios with remarkable efficiency.

In the LIBERO task suites, summarized in Table~\ref{tab: libero ablations}, \gls{mdt} proves to be effective with sparsely labeled data, outperforming the Oracle-BC baseline, which relies on fully labeled demonstrations from LIBERO.
\gls{mdt} not only outperforms the fully language-labeled Transformer Baseline in three out of four challenges but also significantly surpasses the U-Net-based Distill-D policy in all tests, even without auxiliary objectives. 
These outcomes highlight the robustness of our architecture and affirmatively answer Question (I) regarding its efficiency.


\subsection{Evaluation of Masked Generative Foresight}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/evaluation/rss_24_ssl_ablations_legend.pdf}
    \includegraphics[width=\linewidth]{plots/evaluation/mdt_rss_ablations_losses.pdf}
    \caption{Study on the performance of our proposed Masked Generative Foresight Loss and the Contrastive Latent Alignment Loss for our proposed \gls{mdt} policy. 
    We analyse the impact of both auxiliary tasks on the ABCD CALVIN challenge. 
    The results show the average rollout length over 1000 instruction chains averaged over 3 seeds. }
    \label{fig: CALVIN SSL Loss Ablation}
\end{figure}

We next investigate the significance of our auxiliary self-supervised loss functions, specifically the \gls{cla} and \gls{mgf} loss, on \gls{mdt}'s performance. Figure \ref{fig: CALVIN SSL Loss Ablation} shows the performance metrics of the ablated versions with and without these losses.
The inclusion of \gls{mgf} notably enhances \gls{mdt}'s performance on the CALVIN ABCD$\rightarrow$D benchmark, improving average rollout lengths by over $25\%$.
Detailed results supporting the essential role of these auxiliary tasks in \gls{mdt}-V are presented in Table~\ref{tab: MDTV ssl abalations} within the Appendix, showing that \gls{mdt}-V surpasses all baselines with an average rollout length of $4.12$ even in the absence of these two losses.

We further study the impact of \gls{mgf} and \gls{cla} on the LIBERO benchmark (summarized in Table \ref{tab: libero ablations}), where the auxiliary objectives improve \gls{mdt}'s success rates in $4$ out of $5$ test suites, achieving more than a $5.4\%$ increase on average. 
The results of these experiments are summarized in Table \ref{tab: libero ablations}.
Interestingly, we observe a synergistic effect when both losses are applied together. 
However, the LIBERO-Long benchmark does not seem to benefit from either \gls{mgf} or \gls{cla}. 
The demonstrations of the LIBERO-Long benchmark consist of several sub-tasks each with a single high-level description for the entire task.
We hypothesize that this lack of sub-goals prevents the auxiliary losses from providing notable benefits.

To investigate if \gls{mgf} provides a generally beneficial auxiliary objective we integrate it with \gls{mtact} and evaluate the model for the full CALVIN ABCD$\rightarrow$D benchmark, as detailed in \autoref{tab: MT-ACT Ablations}.
\gls{mgf} significantly boosts \gls{mtact}'s average CALVIN performance by $44\%$, without any other modifications to the model or its hyperparameters. 
Similarly to the \gls{mdt} results, \gls{mgf} also enhances the performance of \gls{mtact} to learn better from multimodal goals with few language annotations. 
These positive outcomes for \gls{mdt}, along with its effective application to other transformer-based policies, positively answer research questions (IIa) and (IIb).


\subsection{Real Robot Experiments}


We investigate research question (III), by assessing the ability of \gls{mdt} to learn language-guided manipulation from partially labeled data in a real-world setting.
\gls{mdt} is evaluated on a real-world play kitchen setup with a 7 Degree-of-Freedom Franka Emika Panda Robot.
The setup incorporates two static RGB cameras: one positioned above the kitchen for a bird's-eye view, and another placed on the left side of the robot.
The experiments consist of five distinct tasks involving pick-and-place actions, door opening, and object manipulation.
% We label short sub-sequences with language descriptions to enable language-conditioned manipulation. 
We annotate $20$ sub-sequences of every task with several short language descriptions to create a partially annotated dataset.
To enrich training diversity, some of these descriptions were generated by GPT-4. During training a single description per labeled sub-sequence is sampled. 
The different instructions and the experimental details are summarized in the Appendix~\ref{sec: real world experiments descriptions}. 
Our dataset encompasses around $2.5$ hours of interactive play data.
We evaluated both \gls{mtact} and \gls{mdt} with an action sequence length of $20$, which was optimal for performance on the physical robot.
The models are tested with long-horizon rollouts, requiring the completion of five tasks in sequence. The models were provided $5$ subgoals represented either as images or language descriptions.
The experiments are detailed in \autoref{tab: real robot experiments}. The results highlight \gls{mdt}'s robust performance, particularly in learning from sparse labeling. 
\gls{mdt} was successful in completing $4$ tasks in sequence and showed proficiency in understanding goals expressed through language or images.
The results further emphasise the importance of \gls{mgf} to learn effectively from partially labeled datasets, since the \gls{mdt} variant without this auxiliary objective showed a reduced performance.


\subsection{Additional Ablation Studies}

\textbf{Masked Generative Foresight.}
Next, we study the different design choices of our \gls{mgf} loss and compare them against ablations.
Our primary focus is on assessing the impact of different masking ratios, ranging from $0.5$ to $1$, where $1$ corresponds to a full reconstruction of the initial future image. 
The results indicate that a masking ratio of $0.75$ achieves the best average performance, which is a value commonly used in other masking methods~\cite{karamcheti2023language}.
Thus, we use it as the default masking rate across all experiments in the paper.
Further details of this analysis are provided in Table~\ref{tab: masking rate MGF} in the Appendix.
Additionally, we investigate the ideal foresight distance for \gls{mgf} and evaluate it in two environments.
\gls{mdt} adopts a foresight distance of $v=3$ as this setting consistently delivers strong performance across various scenarios. 
While a higher foresight distance of $v=9$ does exhibit the second-best performance, it is also associated with increased variance in results.
Further results of these investigations are presented in \autoref{tab: prediction horizon MGF} in the Appendix.


\textbf{Transformer Architecture.}
\gls{mdt} is tested against two Diffusion Transformer architectures previously described in~\cite{chi2023diffusionpolicy}.
The ablations are visualized in~\autoref{fig: transformer ablations} of the Appendix. 
These comparisons are conducted on the CALVIN ABCD$\rightarrow$D challenge, with detailed results featured in \ref{tab: MDTV ssl abalations} in the Appendix.
In the first ablation study, we incorporated a noise token as an additional input to the transformer encoder. 
This was done to assess the effect of excluding adaLN noise conditioning.
The second ablation represents the diffusion transformer architecture from~\cite{chi2023diffusionpolicy}, which does not use any encoder module.
\gls{mdt}-V, when trained without any auxiliary objective, achieves an average rollout length of $4.18$. 
The ablation without adaLN conditioning only achieves an average rollout length of $3.58$.
Notably, the complete omission of the transformer encoder led to a significantly lower average rollout length of $1.41$.
The experiments show, that the additional transformer encoder is crucial for diffusion policies to succeed in learning from different goals. 
In addition, separating the denoising process from the encoder and using adaLN conditioning further helps to boost performance and efficiency. 


\subsection{Limitations}

While MDT shows strong performance on learning from multimodal goals, it still has several limitations: 1) While we verify the effectiveness of our method in many tasks, \gls{mgf} and \gls{cla} reduce the performance on LIBERO-Long
2) The Contrastive Loss requires careful filtering of negative goal samples to use its full potential 3) Diffusion Policies require multiple forward passes to generate an action sequence which results in lower inference speed compared to non-diffusion approaches





==> tables/calvin_main_table.tex <==
\begin{table*}
\centering
%\captionsetup{skip=10pt} % Adjust the vertical space as needed
\scalebox{1.4}{
\begin{tabular}{ll|ccccccc}
\toprule
 \multirow{2}{*}{Train$\rightarrow
$Test} &  \multirow{2}{*}{Method} & \multicolumn{6}{c}{No. Instructions in a Row (1000 chains)}  \\
  \cmidrule(lr){3-8}
 &  & 1 & 2 & 3 & 4 & 5 & \textbf{Avg. Len.} \\ \midrule

 \multirow{6}{*}{D$\rightarrow
$D } &  HULC & 82.5\% & 66.8\% & 52.0\% & 39.3\% & 27.5\% & 2.68$\pm$(0.11)  \\
& LAD & 88.7\% & 69.9\% & 54.5\% & 42.7\% & 32.2\% & 2.88$\pm$(0.19) \\
& Distill-D & 86.7\% & 71.5\% & 57.0\% & 45.9\% & 35.6\% & 2.97$\pm$(0.04) \\
% & RoboFlamingo & 77.1\% & 48.3\% & 29.6\% & 16.8\% & 9.9\% & 1.82$\pm$(0.00) \\
& MT-ACT & 88.4\% & 72.2\% & 57.2\% & 44.9\% & 35.3\% & 2.98$\pm$(0.05) \\
& \textbf{MDT (ours)} & \textbf{93.3\%} & \textbf{82.4\%} & \textbf{71.5\%} & \textbf{60.9\%} & \textbf{51.1\%} & \textbf{3.59$\pm$(0.07)}  \\
& \textbf{MDT-V (ours)} & \textbf{93.7\%} & \textbf{83.2\%} & \textbf{71.7\%} & \textbf{60.5\%} & \textbf{50.6\%} & \textbf{3.60$\pm$(0.05)}  \\
\midrule
 \multirow{6}{*}{ABCD$\rightarrow$D } 
& HULC & 88.9\% & 73.3\% & 58.7\% & 47.5\% & 38.3\% & 3.06$\pm$(0.07) \\
& Distill-D & 86.3\% & 72.7\% & 60.1\% & 51.2\% & 41.7\% & 3.16$\pm$(0.06) \\
& MT-ACT & 87.1\% & 69.8\% & 53.4\% & 40.0\% & 29.3\% & 2.80$\pm$(0.03) \\
& RoboFlamingo & 96.4\% & 89.6\% & 82.4\% & 74.0\% & 66.0\% & 4.09$\pm$(0.00) \\
& \textbf{MDT (ours)} & \textbf{97.5\%} & \textbf{92.4\%} & \textbf{87.1\%} & \textbf{81.4\%} & \textbf{74.8\%} & \textbf{4.33$\pm$(0.08)} \\
& \textbf{MDT-V (ours)} & \textbf{98.8\%} & \textbf{95.9\%} & \textbf{91.2\%} & \textbf{86.1\%} & \textbf{79.4\%} & \textbf{4.51$\pm$(0.02)} \\
% \midrule
% \multirow{3}{*}{ABC$\rightarrow
% $D } 
% & HULC & 41.8\% & 16.5\% & 5.7\% & 1.9\% & 1.3\% & 0.67$\pm$(0.10) \\
% & RoboFlamingo & 82.4\% & 61.9\% & 46.6\% & 33.1\% & 23.5\% & 2.47$\pm$(0.00) \\
% & \textbf{MDT (ours)} & \textbf{83.8\%} & \textbf{64.3\%} & \textbf{47.3\%} & \textbf{34.5\%} & \textbf{25.6\%} & \textbf{2.55$\pm$(0.05)} \\
\bottomrule
\end{tabular}}

\caption{
Performance comparison of various policies learned end-to-end on the CALVIN ABCD$\rightarrow
$D and D$\rightarrow$D challenge within the CALVIN benchmark. 
We show the average rollout length to solve $5$ instructions in a row (Avg. Len.) of $1000$ chains. 
Our proposed method MDT and MDT-V significantly outperform all reported baselines averaged over 3 seeds on both datasets and sets a sota performance.
}
\label{tab: CALVIN Long horizon}
\end{table*}

